A Reduced Semantics for Deciding Trace Equivalence

Many privacy-type properties of security protocols can be modelled using trace equivalence properties in suitable process algebras. It has been shown that such properties can be decided for interesting classes of finite processes (i.e., without replication) by means of symbolic execution and constraint solving. However, this does not suffice to obtain practical tools. Current prototypes suffer from a classical combinatorial explosion problem caused by the exploration of many interleavings in the behaviour of processes. M\"odersheim et al. have tackled this problem for reachability properties using partial order reduction techniques. We revisit their work, generalize it and adapt it for equivalence checking. We obtain an optimisation in the form of a reduced symbolic semantics that eliminates redundant interleavings on the fly. The obtained partial order reduction technique has been integrated in a tool called APTE. We conducted complete benchmarks showing dramatic improvements.

==> bpicture.tex <==
%\renewcommand{\t}{t}

\setlength{\fboxsep}{10pt}
\setlength{\fboxrule}{1pt}
%\newcommand*\mystrut[1]{\vrule width0pt height0pt depth#1\relax}

\newcommand{\printint}[0]{ %%%%%%%%%%%%%%% Intermediate
  \fbox{
    \begin{minipage}{10pt}\small
      $\sint{\ }$\\[13pt]
      $\eint$
    \end{minipage}
  }
}
\newcommand{\printcomp}[0]{ %%%%%%%%%%%%%%% Compressed
  \fbox{
    \begin{minipage}{10pt}\small
      $\sintc{\ }$\\[13pt]
      $\eintc$
    \end{minipage}
  }
}
\newcommand{\printcompsymb}[0]{ %%%%%%%%%%%%%%% Compressed symbolic
  \fbox{
    \begin{minipage}{10pt}\small
      $\ssymc{\ \ \ }$\\[13pt]
      $\esymc$
    \end{minipage}
  }
}
\newcommand{\printred}[0]{      %Reduced symbolic
  %%%%%%%%%%% Reduced
  \fbox{
    \begin{minipage}{25pt}\small
      ${\hspace{-5pt}\ssymc{\ }+}\\ \AllDep{\cdot}$\\[1pt]
      $\esymdff$
    \end{minipage}
  }
}
\newcommand{\printapte}[0]{      % Apte
  %%%%%%%%%%% Reduced
  \fbox{
    \begin{minipage}{10pt}\small
      $\ssyma{\ }$\\[13pt]
      $\eqapte$
    \end{minipage}
  }
}
\newcommand{\printaptecomp}[0]{      % Apte comp
  %%%%%%%%%%% Reduced
  \fbox{
    \begin{minipage}{10pt}\small
      $\ssymac{\ }$\\[13pt]
      $\eqaptec$
    \end{minipage}
  }
}
\newcommand{\printaptered}[0]{      % Apte red
  %%%%%%%%%%% Reduced
  \fbox{
    \begin{minipage}{10pt}\small
      $\ssymad{\ }$\\[9pt]
      $\eqapted$
    \end{minipage}
  }
}
\setlength{\fboxsep}{10pt}
\setlength{\fboxrule}{1pt}
%\newcommand*\mystrut2[1]{\vrule width0pt height0pt depth#1\relax}
\newcommand{\alert}[1]{{#1}}
\definecolor{vert2}{rgb}{0,0,0}

\begin{figure}[t]
  \centering
   \begin{tabular}[h]{l}
      \hspace{-25pt}
      $\printint
     \underset
     {\alert{\text{Theorem 1}:\  \eint = \eintc}}
     {\xRightarrow{\color{vert2}{\text{\bf Compression\ }}}}
      \printcomp

      \underset
      {\text{Theorem 2:}\  \eintc=\esymc}
      {\xRightarrow{{\text{Symbolic\ }}}}

      \printcompsymb

      \underset
      {\alert{\text{Corollary 2}:\  \esymc = \esymdff}}
      {\xRightarrow{\color{vert2}{\text{\bf Reduction\ }}}}

      \printred
     $
\\[-5pt]
      $
\phantom{     \printcomp}
     \phantom{
     \underset
     {\alert{\text{Corollary 1}:\ \eint = \eintc}}
     {\xRightarrow{\color{vert2}{\text{\bf Compression}}}}}
\phantom{      \printcomp}

     \phantom{
     \underset
     {\text{Classical:}\ \eintc=\esymc}
     {\xRightarrow{{\text{\bf Symbolic}}}}}

\hspace{-78pt}
\text{\scriptsize{Theorem 5: }}{\scriptscriptstyle \esymc=\eqaptec}
\ \bigg\Downarrow{}

\hspace{35pt}

\text{\scriptsize{Theorem 6: }}{\scriptscriptstyle \esymdff=\eqapted}
\ \bigg\Downarrow{}
     $
\\[-5pt]
      $
\phantom{     \printcomp}
     \phantom{
     \underset
     {\alert{\text{Corollary 1}:\ \eint = \eintc}}
     {\xRightarrow{\color{vert2}{\text{\bf Compression}}}}}
\phantom{      \printcomp}


     \phantom{
     \underset
     {\text{Classical:}\ \eintc=\esymc}
     {\xRightarrow{{\text{\bf Symbolic}}}}}

\hspace{-165pt}
\text{Semantics of the tool \apte}
\left\lbrace
\hspace{25pt}

\hspace{-8pt}
     \printaptecomp


     \phantom{
     \underset
     {\alert{\text{Corollary 2}:\ \esymc = \eintd}}
     {\xRightarrow{\color{vert2}{\text{\bf Reduction}}}}}

\hspace{15pt}
      \printaptered
\hspace{25pt}\right\rbrace
     $

    \end{tabular}


\lucca{TODO: la figure discutee}
%  \caption{Big Picture of our approach: from the concrete semantics $\rightarrow$ (and equivalence $\eint$)
%    to our optimised semantics and their respective equivalences in theory and in the tool \apte}
\caption{Overview of our approach}
 \label{fig:bpicture}
\end{figure}


==> tikzlibrarynode-families.code.tex <==
\let\tikz@lib@nf@textheight\relax
\let\tikz@lib@nf@textdepth\relax
\let\tikz@lib@nf@textwidth\relax
\tikzset{
  Minimum Width/.code={%
    \pgfutil@ifundefined{\pgfpictureid @#1@width}{}{%
      \tikzset{/tikz/minimum width/.expand twice=+\csname\pgfpictureid @#1@width\endcsname}%
    }%
    \tikz@addmode{\pgfmathsetlengthmacro\tikz@lib@nf@outerxsep{\pgfkeysvalueof{/pgf/outer xsep}}\global\let\tikz@lib@nf@outerxsep\tikz@lib@nf@outerxsep}%
    \tikzset{
      prefix after command={%
        \pgfextra
          \pgfinterruptpath
            \pgfsettransform{\csname pgf@sh@nt@\tikzlastnode\endcsname}%
            \pgfpointanchor{\tikzlastnode}{east}%
            \pgf@xa=\pgf@x \pgf@ya=\pgf@y
            \pgfpointanchor{\tikzlastnode}{west}%
            \advance\pgf@xa-\pgf@x
            \advance\pgf@ya-\pgf@y
            \pgfmathveclen@{\pgf@sys@tonumber\pgf@xa}{\pgf@sys@tonumber\pgf@ya}%
            \pgf@x\pgfmathresult pt\relax
            \advance\pgf@x-\tikz@lib@nf@outerxsep
            \advance\pgf@x-\tikz@lib@nf@outerxsep
            \pgfutil@ifundefined{\pgfpictureid @#1@width}{%
              \expandafter\xdef\csname\pgfpictureid @#1@width\endcsname{\the\pgf@x}%
            }{%
              \expandafter\ifdim\csname\pgfpictureid @#1@width\endcsname<\pgf@x
                \expandafter\xdef\csname\pgfpictureid @#1@width\endcsname{\the\pgf@x}%
              \fi
            }%
            \expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter
            \tikz@atend@picture\expandafter\expandafter\expandafter{\expandafter\tikz@atend@picture\expandafter\tikz@lib@nf@save\expandafter{\pgfpictureid}{#1}{width}{width}}
          \endpgfinterruptpath
        \endpgfextra
      }%
    }%
  },
  Minimum Height/.code={%
    \pgfutil@ifundefined{\pgfpictureid @#1@height}{}{%
      \tikzset{/tikz/minimum height/.expand twice=+\csname\pgfpictureid @#1@height\endcsname}%
    }%
    \tikz@addmode{\pgfmathsetlengthmacro\tikz@lib@nf@outerysep{\pgfkeysvalueof{/pgf/outer ysep}}\global\let\tikz@lib@nf@outerysep\tikz@lib@nf@outerysep}%
    \tikzset{
      prefix after command={%
        \pgfextra
          \pgfinterruptpath
            \pgfsettransform{\csname pgf@sh@nt@\tikzlastnode\endcsname}%
            \pgfpointanchor{\tikzlastnode}{north}%
            \pgf@xa=\pgf@x \pgf@ya=\pgf@y
            \pgfpointanchor{\tikzlastnode}{south}%
            \advance\pgf@xa-\pgf@x
            \advance\pgf@ya-\pgf@y
            \pgfmathveclen@{\pgf@sys@tonumber\pgf@xa}{\pgf@sys@tonumber\pgf@ya}%
            \pgf@x\pgfmathresult pt\relax
            \advance\pgf@x-\tikz@lib@nf@outerysep
            \advance\pgf@x-\tikz@lib@nf@outerysep
            \pgfutil@ifundefined{\pgfpictureid @#1@height}{%
              \expandafter\xdef\csname\pgfpictureid @#1@height\endcsname{\the\pgf@x}%
            }{%
              \expandafter\ifdim\csname\pgfpictureid @#1@height\endcsname<\pgf@x
                \expandafter\xdef\csname\pgfpictureid @#1@height\endcsname{\the\pgf@x}%
              \fi
            }%
            \expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter
            \tikz@atend@picture\expandafter\expandafter\expandafter{\expandafter\tikz@atend@picture\expandafter\tikz@lib@nf@save\expandafter{\pgfpictureid}{#1}{height}{height}}
          \endpgfinterruptpath
        \endpgfextra
      }%
    }%
  },
  Minimum Size/.style={
    Minimum Height={#1},
    Minimum Width={#1}},
  Text Height/.code=\edef\tikz@lib@nf@textheight{#1},
  Text Depth/.code= \edef\tikz@lib@nf@textdepth{#1},
  Text Width/.code=%
    \edef\tikz@lib@nf@textwidth{#1}%
    \pgfutil@ifundefined{\pgfpictureid @#1@textwidth}{}{%
      \tikzset{text width/.expand twice=+\csname\pgfpictureid @#1@textwidth\endcsname}%
    }%
}

\def\tikz@lib@nf@text@#1#2#3{%
  \expandafter\ifx\csname tikz@lib@nf@#3\endcsname\relax\else
    \ifx#1\wd\def\tikz@temp{@}\else\let\tikz@temp\pgfutil@empty\fi
    \expandafter\ifx\csname tikz@lib@nf@#3\tikz@temp\endcsname\pgfutil@empty\else
      \pgfutil@ifundefined{\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp}{%
        \expandafter\xdef\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp\endcsname{\the#1#2}%
      }{%
        \ifdim\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp\endcsname<#1#2
          \expandafter\xdef\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp\endcsname{\the#1#2}%
        \else
          \ifx#1\wd\else
            #1#2=\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\endcsname\relax
          \fi
        \fi
      }%
      \edef\tikz@temp{\noexpand\tikz@lib@nf@save{\pgfpictureid}{\csname tikz@lib@nf@#3\endcsname}{#3}{#3\tikz@temp}}%
      \expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter
      \tikz@atend@picture\expandafter\expandafter\expandafter{\expandafter\tikz@atend@picture\tikz@temp}%
    \fi
  \fi
}
%%% Redefinition
\def\tikz@fig@continue{%
    \ifx\tikz@text@width\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@width}%
      \wd\pgfnodeparttextbox=\pgf@x%
    \fi%
    \ifx\tikz@text@height\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@height}%
      \ht\pgfnodeparttextbox=\pgf@x%
    \fi%
    \ifx\tikz@text@depth\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@depth}%
      \dp\pgfnodeparttextbox=\pgf@x%
    \fi%
    %
    %
    %
    \tikz@lib@nf@text@\ht\pgfnodeparttextbox{textheight}%
    \tikz@lib@nf@text@\dp\pgfnodeparttextbox{textdepth}%
    \tikz@lib@nf@text@\wd\pgfnodeparttextbox{textwidth}%
    %
    % Node transformation
    %
    \tikz@node@transformations
    %
    \setbox\tikz@figbox=\hbox{%
      \setbox\pgfutil@tempboxa=\copy\tikz@figbox%
      \unhbox\pgfutil@tempboxa%
      \hbox{{%
          \pgfinterruptpath%
            \pgfscope%
              \tikz@options%
              \setbox\tikz@figbox=\box\pgfutil@voidb@x%
              \pgfmultipartnode{\tikz@shape}{\tikz@anchor}{\tikz@fig@name}{%
                \pgfutil@tempdima=\pgflinewidth%
                {\begingroup\tikz@finish}%
                \global\pgflinewidth=\pgfutil@tempdima%
              }%
            \endpgfscope
          \endpgfinterruptpath%
      }}%
    }%
    %
    \tikz@alias%
    \tikz@node@finish%
}
\def\tikz@lib@nf@save#1#2#3#4{%
  \pgfutil@ifundefined{#1@#2@#3@done}{%
    \expandafter\let\csname#1@#2@#3@done\endcsname\pgfutil@empty%
    \immediate\write\pgfutil@auxout{\noexpand\expandafter\noexpand\gdef\noexpand\csname#1@#2@#3\endcsname{\csname#1@#2@#4\endcsname}}
  }{}%
}
\endinput


==> tikzlibrarypositioning-plus.code.tex <==
% This is the TikZ library positioning-plus
% Load with \usetikzlibrary{positioning-plus}
%
% This small library extends TikZ options like 'above', 'left' or 'below right'
% so that they can be used with an optional prefixed factor seperated by ':' (colon)
%
% The option 'left=.5:of somenode' will place
% a new node .5cm (default 'node distance' is '1cm and 1cm') left to (somenode).
% The option 'above right=.2 and .7:of someothernode' will place
% a new node .2cm above and .7cm right of (someothernode).
%
% Additional the options 'xshift*' and 'yshift*' add an additional shift
% as a factor of 'node distance'
% Inspired by http://tex.stackexchange.com/a/117610/16595

\usetikzlibrary{positioning}
\usetikzlibrary{fit}

\pgfdeclaregenericanchor{corner south east}{%
  \pgf@sh@reanchor{#1}{south}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{east}}%
  \pgf@y\pgf@ya
}
\pgfdeclaregenericanchor{corner north east}{%
  \pgf@sh@reanchor{#1}{north}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{east}}%
  \pgf@y\pgf@ya
}
\pgfdeclaregenericanchor{corner south west}{%
  \pgf@sh@reanchor{#1}{south}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{west}}%
  \pgf@y\pgf@ya
}
\pgfdeclaregenericanchor{corner north west}{%
  \pgf@sh@reanchor{#1}{north}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{west}}%
  \pgf@y\pgf@ya
}

\tikzset{corner above left/.code=\tikz@lib@place@handle@{#1}{corner south east}{-1}{1}{corner north west}{0.707106781}}
\tikzset{corner above right/.code=\tikz@lib@place@handle@{#1}{corner south west}{1}{1}{corner north east}{0.707106781}}
\tikzset{corner below left/.code=\tikz@lib@place@handle@{#1}{corner north east}{-1}{-1}{corner south west}{0.707106781}}
\tikzset{corner below right/.code=\tikz@lib@place@handle@{#1}{corner north west}{1}{-1}{corner south east}{0.707106781}}

\tikzset{corner north left/.code =\tikz@lib@place@handle@{#1}{corner north east}{-1}{0}{corner north west}{1}}
\tikzset{corner north right/.code=\tikz@lib@place@handle@{#1}{corner north west}{1}{0}{corner north east}{1}}
\tikzset{corner south left/.code =\tikz@lib@place@handle@{#1}{corner south east}{-1}{0}{corner south west}{1}}
\tikzset{corner south right/.code=\tikz@lib@place@handle@{#1}{corner south west}{1}{0}{corner south east}{1}}

\tikzset{corner west above/.code =\tikz@lib@place@handle@{#1}{corner south west}{0}{1}{corner north west}{1}}
\tikzset{corner west below/.code=\tikz@lib@place@handle@{#1}{corner north west}{0}{-1}{corner south west}{1}}
\tikzset{corner east above/.code =\tikz@lib@place@handle@{#1}{corner south east}{0}{1}{corner north east}{1}}
\tikzset{corner east below/.code=\tikz@lib@place@handle@{#1}{corner north east}{0}{-1}{corner south east}{1}}

\tikzset{north left/.code =\tikz@lib@place@handle@{#1}{north east}{-1}{0}{north west}{1}}
\tikzset{north right/.code=\tikz@lib@place@handle@{#1}{north west}{1}{0}{north east}{1}}
\tikzset{south left/.code =\tikz@lib@place@handle@{#1}{south east}{-1}{0}{south west}{1}}
\tikzset{south right/.code=\tikz@lib@place@handle@{#1}{south west}{1}{0}{south east}{1}}

\tikzset{west above/.code =\tikz@lib@place@handle@{#1}{south west}{0}{1}{north west}{1}}
\tikzset{west below/.code=\tikz@lib@place@handle@{#1}{north west}{0}{-1}{south west}{1}}
\tikzset{east above/.code =\tikz@lib@place@handle@{#1}{south east}{0}{1}{north east}{1}}
\tikzset{east below/.code=\tikz@lib@place@handle@{#1}{north east}{0}{-1}{south east}{1}}

\newif\ifqrr@tikz@lib@place@postransform
\tikzset{node distance transformation/.is if=qrr@tikz@lib@place@postransform}
\def\tikz@lib@place@handle@@#1#2#3#4{%
  \pgfutil@in@{of }{#1}%
  \ifpgfutil@in@%
    \tikz@lib@place@of#1\tikz@stop{#4}%
  \else%
    \edef\tikz@lib@place@nums{#1}%
  \fi%
  \ifx\tikz@lib@place@nums\pgfutil@empty%
    % Ok, nothing to do, we have set the anchor and we are happy...
  \else%
    \expandafter\tikz@lib@place@parse@nums\expandafter{\tikz@lib@place@nums}%
    \pgf@x=#2\pgf@x%
    \pgf@y=#3\pgf@y%
    \ifqrr@tikz@lib@place@postransform
      \pgf@pos@transform{\pgf@x}{\pgf@y}% change from original
    \fi
    \edef\tikz@lib@pos@call{\noexpand\pgftransformshift{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  \fi%
}

\def\tikz@lib@place@handle@#1#2#3#4#5#6{%
  \pgfutil@in@{:}{#1}%
  \ifpgfutil@in@
    \tikz@lib@place@handle@qrr@#1\tikz@stop
    \ifx\pgf@temp\pgfutil@empty
      \let\pgf@temp\tikz@node@distance
    \fi
    \pgfmathsetmacro\pgf@tempa{(\pgf@tempa)*#4}%
    \pgfmathsetmacro\pgf@tempb{(\pgf@tempb)*#3}%
    \edef\pgf@marshal{\noexpand\tikz@lib@place@handle@{\pgf@temp}{#2}{\pgf@tempb}{\pgf@tempa}{#5}{#6}}%
    \pgf@marshal
  \else
    \def\tikz@anchor{#2}%
    \let\tikz@do@auto@anchor=\relax%
    \edef\tikz@temp{#1}%
    \def\tikz@lib@place@single@factor{#6}%
    \expandafter\tikz@lib@place@handle@@\expandafter{\tikz@temp}{#3}{#4}{#5}%
  \fi
}
\def\tikz@lib@place@handle@qrr@#1:#2\tikz@stop{%
  \pgfutil@in@{and}{#1}%
  \ifpgfutil@in@
    \tikz@lib@place@handle@qrr@@#1\tikz@stop
  \else
    \tikz@lib@place@handle@qrr@@#1and#1\tikz@stop
  \fi
  \def\pgf@temp{#2}%
}
\def\tikz@lib@place@handle@qrr@@#1and#2\tikz@stop{%
  \def\pgf@tempa{#1}%
  \def\pgf@tempb{#2}%
}
\def\qrr@xyshift@starred#1#2#3{
  \edef\tikz@marshal{\noexpand\pgfutil@in@{and}{\tikz@node@distance}}%
  \tikz@marshal
  \ifpgfutil@in@
    \expandafter\tikz@lib@place@handle@qrr@@\tikz@node@distance\tikz@stop
  \else
    \let#3\tikz@node@distance
  \fi
  \pgfmathparse{(#1)*#3}%
  \ifpgfmathunitsdeclared
    \if#2x%
      \pgftransformshift{\pgfqpoint{\pgfmathresult pt}{0pt}}%
    \else
      \pgftransformshift{\pgfqpoint{0pt}{\pgfmathresult pt}}%
    \fi
  \else
    \ifx#2x
      \pgf@process{\pgfqpointxy{\pgfmathresult}{0}}%
    \else
      \pgf@process{\pgfqpointxy{0}{\pgfmathresult}}%
    \fi
    \pgftransformshift{\pgfqpoint{\pgf@x}{\pgf@y}}%
  \fi}
\tikzset{
  xshift*/.code=\qrr@xyshift@starred{#1}x\pgf@tempb,
  yshift*/.code=\qrr@xyshift@starred{#1}y\pgf@tempa,
}

\def\pgfutil@firstofmany#1#2\pgf@stop{#1}
\def\pgfutil@secondofmany#1#2\pgf@stop{#2}
\def\tikz@lib@place@of@#1#2#3{%
  \def\pgf@tempa{fit bounding box}%
  \edef\pgf@temp{\expandafter\pgfutil@firstofmany#2\pgf@stop}
  \if\pgf@temp(%
    \tikz@lib@place@fit@scan{#2}{0}%
  \else\if\pgf@temp|
      \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{1}%
    \else\ifx\pgf@temp\tikz@activebar
        \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{1}%
      \else\if\pgf@temp-
          \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{2}%
        \else\if\pgf@temp+
            \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{3}%
          \else
            \def\pgf@tempa{#2}%
          \fi
        \fi
      \fi
    \fi
  \fi
  \expandafter\tikz@scan@one@point\expandafter\tikz@lib@place@remember\expandafter(\pgf@tempa)%
  \iftikz@shapeborder%
    % Ok, this is relative to a border.
    \iftikz@lib@ignore@size%
      \edef\tikz@node@at{\noexpand\pgfpointanchor{\tikz@shapeborder@name}{center}}%
      \def\tikz@anchor{center}%
    \else%
      \edef\tikz@node@at{\noexpand\pgfpointanchor{\tikz@shapeborder@name}{#3}}%
    \fi%
  \fi%
  \edef\tikz@lib@place@nums{#1}%
}
\def\tikz@lib@place@fit@scan#1#2{
  \pgf@xb=-16000pt\relax%
  \pgf@xa=16000pt\relax%
  \pgf@yb=-16000pt\relax%
  \pgf@ya=16000pt\relax%
  \if\pgfutil@firstofmany#1\pgf@stop(%
    \tikz@lib@fit@scan#1\pgf@stop%
  \else
    \tikz@lib@fit@scan(#1)\pgf@stop
  \fi
  \ifdim\pgf@xa>\pgf@xa
    % shouldn't happen
  \else
     \expandafter\def\csname pgf@sh@ns@fit bounding box\endcsname{rectangle}%
     \expandafter\edef\csname pgf@sh@np@fit bounding box\endcsname{%
       \def\noexpand\southwest{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
       \def\noexpand\northeast{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
     }%
     \expandafter\def\csname pgf@sh@nt@fit bounding box\endcsname{{1}{0}{0}{1}{0pt}{0pt}}%
     \expandafter\def\csname pgf@sh@pi@fit bounding box\endcsname{\pgfpictureid}%
     \ifcase#2\relax
     \or % 1 = vertical
       \pgf@y=\pgf@yb%
       \advance\pgf@y by-\pgf@ya%
       \edef\pgf@marshal{\noexpand\tikzset{minimum height={\the\pgf@y-2*(\noexpand\pgfkeysvalueof{/pgf/outer ysep})}}}%
       \pgf@marshal
     \or % 2 = horizontal
       \pgf@x=\pgf@xb%
       \advance\pgf@x by-\pgf@xa%
       \edef\pgf@marshal{\noexpand\tikzset{minimum width={\the\pgf@x-2*(\noexpand\pgfkeysvalueof{/pgf/outer xsep})}}}%
       \pgf@marshal
     \or % 3 = both directions
       \pgf@y=\pgf@yb%
       \advance\pgf@y by-\pgf@ya%
       \pgf@x=\pgf@xb%
       \advance\pgf@x by-\pgf@xa%
       \edef\pgf@marshal{\noexpand\tikzset{minimum height={\the\pgf@y-2*(\noexpand\pgfkeysvalueof{/pgf/outer ysep})},minimum width={\the\pgf@x-2*(\noexpand\pgfkeysvalueof{/pgf/outer xsep})}}}%
       \pgf@marshal
     \fi
  \fi
}
\tikzset{
  fit bounding box/.code={\tikz@lib@place@fit@scan{#1}{0}},
  span vertical/.code={\tikz@lib@place@fit@scan{#1}{1}},
  span horizontal/.code={\tikz@lib@place@fit@scan{#1}{2}},
  span/.code={\tikz@lib@place@fit@scan{#1}{3}}}

\pgfmathdeclarefunction{x_node_dist}{0}{%
  \begingroup
    \edef\pgfmath@temp{\noexpand\pgfutil@in@{and}{\tikz@node@distance}}%
    \pgfmath@temp\ifpgfutil@in@
      \expandafter\tikz@lib@place@handle@qrr@@\tikz@node@distance\tikz@stop
    \else
      \edef\pgfmath@temp{\tikz@node@distance and\tikz@node@distance}%
      \expandafter\tikz@lib@place@handle@qrr@@\pgfmath@temp\tikz@stop
    \fi
    \pgfmathparse{\pgf@tempb}%
    \pgfmath@smuggleone\pgfmathresult
  \endgroup
}
\pgfmathdeclarefunction{y_node_dist}{0}{%
  \begingroup
    \edef\pgfmath@temp{\noexpand\pgfutil@in@{and}{\tikz@node@distance}}%
    \pgfmath@temp\ifpgfutil@in@
      \expandafter\tikz@lib@place@handle@qrr@@\tikz@node@distance\tikz@stop
    \else
      \edef\pgfmath@temp{\tikz@node@distance and\tikz@node@distance}%
      \expandafter\tikz@lib@place@handle@qrr@@\pgfmath@temp\tikz@stop
    \fi
    \pgfmathparse{\pgf@tempa}%
    \pgfmath@smuggleone\pgfmathresult
  \endgroup
}
%\tikzdeclarecoordinatesystem{node distance}{%
%  \tikz@cs@nd#1\tikz@stop}
%\def\tikz@cs@nd#1,#2\tikz@stop{%
%  \def\qrr@xyshift@starred@action##1{\pgftransformshift{##1}}%
%  \qrr@xyshift@starred{#1}x\pgf@tempb
%  \qrr@xyshift@starred{#2}y\pgf@tempa}
\endinput

